Towards Explainable Conversational Recommender Systems

Explanations in conventional recommender systems have demonstrated benefits in helping the user understand the rationality of the recommendations and improving the system's efficiency, transparency, and trustworthiness. In the conversational environment, multiple contextualized explanations need to be generated, which poses further challenges for explanations. To better measure explainability in conversational recommender systems (CRS), we propose ten evaluation perspectives based on concepts from conventional recommender systems together with the characteristics of CRS. We assess five existing CRS benchmark datasets using these metrics and observe the necessity of improving the explanation quality of CRS. To achieve this, we conduct manual and automatic approaches to extend these dialogues and construct a new CRS dataset, namely Explainable Recommendation Dialogues (E-ReDial). It includes 756 dialogues with over 2,000 high-quality rewritten explanations. We compare two baseline approaches to perform explanation generation based on E-ReDial. Experimental results suggest that models trained on E-ReDial can significantly improve explainability while introducing knowledge into the models can further improve the performance. GPT-3 in the in-context learning setting can generate more realistic and diverse movie descriptions. In contrast, T5 training on E-ReDial can better generate clear reasons for recommendations based on user preferences. E-ReDial is available at https://github.com/Superbooming/E-ReDial.

==> tables/dataset_info.tex <==
\begin{table}[!t]
\small
\centering
\setlength\tabcolsep{1.5pt}
\caption{
Statistic of sampled dialogues in different datasets. 
}
\label{table:datasets_statistic}
\begin{tabular}{l rrrrr}

\toprule

\textbf{Datasets} 
& \textbf{ReDial}
& \textbf{TG-ReDial}
& \textbf{DuRecDial}
& \textbf{INSPIRED}
& \textbf{OpenDialKG} \\

\midrule

Language
& English & Chinese & Chinese & English & English \\         
\#Dialogues
& 50 & 50 & 50 & 50 & 50 \\

\#Uttrances
& 891 & 656 & 830 & 1750 & 347 \\

Avg\# Turns
& 17.82 & 13.12 & 16.60 & 35.00 & 6.54 \\

\bottomrule
\end{tabular}
\end{table}


==> tables/eredial_info.tex <==
\begin{table}[!t]
\small
\centering
\setlength\tabcolsep{8pt}
\caption{
The statistics and evaluation results of E-ReDial.
}
\label{table:eredial_info}
\begin{tabular}{l r}
\toprule
\multicolumn{2}{l}{\textbf{Statistics}} 
\\

\midrule

\#Dialogs & 756 \\

\#Utterances & 12,003 \\

Avg\# Turns & 15.9\\

\#Rewritten Explanations & 2,058 \\

Avg\# Tokens in Explanations & 79.2 \\

\midrule

\multicolumn{2}{l}{\textbf{Evaluation Results}} 
\\

\midrule

Effectiveness & 2.96 \\

Efficiency & 2.95 \\

Persuasiveness & 2.92 \\

Transparency & 2.97 \\

Scrutability & 2.95 \\

Trust & 2.89 \\

Satisfaction & 2.92 \\

Representativeness & 2.99 \\

Reasonability & 2.99 \\

Coherence & 2.99 \\

Overall & 4.04 \\

\bottomrule
\end{tabular}
\end{table}

==> tables/results_decoding.tex <==
\begin{table}[!t]
\small
\centering
\setlength\tabcolsep{5pt}
\caption{
Performance for response generation among different decoding methods in \emph{Test-Full}. Bold face indicates the best result in terms of the corresponding metric.
}
\label{table:results_decoding}
\begin{tabular}{l cccccc}
\toprule
& F1  & B2 & B4 & MT & D2 & D3 
\\ 

\midrule
T5-Base+KG
& 26.01 & 7.89 & 4.10 & 16.29 & 47.60 & 59.44
\\

\midrule

+ Beam ($b$=3)
& \textbf{26.07} & \textbf{8.57} & \textbf{4.67} & \textbf{16.93} & 48.16 & 59.55
\\

+ Temperature ($t$=0.5)
& 24.93 & 7.41 & 3.82 & 15.91 & 48.89 & 62.35
\\

+ Top-$k$ ($k$=30)
& 20.90 & 5.63 & 2.78 & 13.16 & \textbf{54.45} & \textbf{70.62}
\\

+ Nucleus ($p$=0.9)
& 22.22 & 5.99 & 2.77 & 14.12 & 51.91 & 67.08
\\

+ Typical ($p$=0.9)
& 23.81 & 7.05 & 3.60 & 14.94 & 52.04 & 67.31
\\


\bottomrule
\end{tabular}
\end{table}








